Detection of Edges in Spectral Data II. Nonlinear Enhancement

We discuss a general framework for recovering edges in piecewise smooth functions with finitely many jump discontinuities, where $[f](x):=f(x+)-f(x-) \neq 0$. Our approach is based on two main aspects--localization using appropriate concentration kernels and separation of scales by nonlinear enhancement. To detect such edges, one employs concentration kernels, $K_\epsilon(\cdot)$, depending on the small scale $\epsilon$. It is shown that odd kernels, properly scaled, and admissible (in the sense of having small $W^{-1,\infty}$-moments of order ${\cal O}(\epsilon)$) satisfy $K_\epsilon*f(x) = [f](x) +{\cal O}(\epsilon)$, thus recovering both the location and amplitudes of all edges.As an example we consider general concentration kernels of the form $K^\sigma_N(t)=\sum\sigma(k/N)\sin kt$ to detect edges from the first $1/\epsilon=N$ spectral modes of piecewise smooth f's. Here we improve in generality and simplicity over our previous study in [A. Gelb and E. Tadmor, Appl. Comput. Harmon. Anal., 7 (1999), pp. 101-135]. Both periodic and nonperiodic spectral projections are considered. We identify, in particular, a new family of exponential factors, $\sigma^{exp}(\cdot)$, with superior localization properties. The other aspect of our edge detection involves a nonlinear enhancement procedure which is based on separation of scales between the edges, where $K_\epsilon*f(x)\sim [f](x) \neq 0$, and the smooth regions where $K_\epsilon*f = {\cal O}(\epsilon) \sim 0$. Numerical examples demonstrate that by coupling concentration kernels with nonlinear enhancement one arrives at effective edge detectors.

==> mathmacro.tex <==
\newcommand{\nwc}{\newcommand}
\newcommand{\nwt}{\newtheorem}
\nwc{\ba}{\begin{array}}
\nwc{\be}{\begin{equation}}
\nwc{\bdm}{\begin{displaymath}}
\nwc{\beq}{\begin{eqnarray}}
\nwc{\beqn}{\begin{eqnarray*}}
\nwc{\beqast}{\begin{eqnarray*}}
\nwc{\bm}{\boldmath}

\nwc{\bs}{\begin{section}}
\nwc{\bss}{\begin{subsection}}
\nwc{\es}{\end{section}}
\nwc{\ess}{\end{subsection}}

\nwc{\bt}{\begin{theorem}}
\nwc{\et}{\end{theorem}}

\nwc{\m}{\mbox}
\nwc{\BBox}{\quad \rule{.1in}{.1in}}
%\nwc{\Box}{\quad \parbox[b]}
\nwc{\ubm}{\unboldmath}

\nwc{\eps}{\varepsilon}
\nwc{\hf}{\frac{1}{2}}

\nwc{\bma}{\m{\bm $a$ \ubm}}
\nwc{\bmma}{\m{\bm $a$\ubm}}
\nwc{\bmb}{\m{\bm $b$ \ubm}}
\nwc{\bmmb}{\m{\bm $b$\ubm}}
\nwc{\bmc}{\m{\bm $c$ \ubm}}
\nwc{\bmmc}{\m{\bm $c$\ubm}}
\nwc{\bmd}{\m{\bm $d$ \ubm}}
\nwc{\bmmd}{\m{\bm $d$\ubm}}
\nwc{\bme}{\m{\bm $e$ \ubm}}
\nwc{\bmme}{\m{\bm $e$\ubm}}
\nwc{\bmf}{\m{\bm $f$ \ubm}}
\nwc{\bmmf}{\m{\bm $f$\ubm}}
\nwc{\bmg}{\m{\bm $g$ \ubm}}
\nwc{\bmmg}{\m{\bm $g$\ubm}}
\nwc{\bmh}{\m{\bm $h$ \ubm}}
\nwc{\bmmh}{\m{\bm $h$\ubm}}
\nwc{\bmi}{\m{\bm $i$ \ubm}}
\nwc{\bmmi}{\m{\bm $i$\ubm}}
\nwc{\bmj}{\m{\bm $j$ \ubm}}
\nwc{\bmmj}{\m{\bm $j$\ubm}}
\nwc{\bmk}{\m{\bm $k$ \ubm}}
\nwc{\bmmk}{\m{\bm $k$\ubm}}
\nwc{\bml}{\m{\bm $l$ \ubm}}
\nwc{\bmml}{\m{\bm $l$\ubm}}
\nwc{\bmm}{\m{\bm $m$ \ubm}}
\nwc{\bmmm}{\m{\bm $m$\ubm}}
\nwc{\bmn}{\m{\bm $n$ \ubm}}
\nwc{\bmmn}{\m{\bm $n$\ubm}}
\nwc{\bmo}{\m{\bm $o$ \ubm}}
\nwc{\bmmo}{\m{\bm $o$\ubm}}
\nwc{\bmp}{\m{\bm $p$ \ubm}}
\nwc{\bmmp}{\m{\bm $p$\ubm}}
\nwc{\bmq}{\m{\bm $q$ \ubm}}
\nwc{\bmmq}{\m{\bm $q$\ubm}}
\nwc{\bmr}{\m{\bm $r$ \ubm}}
\nwc{\bmmr}{\m{\bm $r$\ubm}}
\nwc{\bms}{\m{\bm $s$ \ubm}}
\nwc{\bmms}{\m{\bm $s$\ubm}}
\nwc{\bmt}{\m{\bm $t$ \ubm}}
\nwc{\bmmt}{\m{\bm $t$\ubm}}
\nwc{\bmu}{\m{\bm $u$ \ubm}}
\nwc{\bmmu}{\m{\bm $u$\ubm}}
\nwc{\bmv}{\m{\bm $v$ \ubm}}
\nwc{\bmmv}{\m{\bm $v$\ubm}}
\nwc{\bmw}{\m{\bm $w$ \ubm}}
\nwc{\bmmw}{\m{\bm $w$\ubm}}
\nwc{\bmx}{\m{\bm $x$ \ubm}}
\nwc{\bmmx}{\m{\bm $x$\ubm}}
\nwc{\bmy}{\m{\bm $y$ \ubm}}
\nwc{\bmmy}{\m{\bm $y$\ubm}}
\nwc{\bmz}{\m{\bm $z$ \ubm}}
\nwc{\bmmz}{\m{\bm $z$\ubm}}

\nwc{\bmX}{\m{\bm $X$\ubm}}
\nwc{\bmR}{\m{\bm $R$\ubm}}
\nwc{\bmU}{\m{\bm $U$\ubm}}
\nwc{\bmF}{\m{\bm $F$\ubm}}


\nwc{\bmtheta}{\m{\bm $\theta$\ubm}}
\nwc{\bmomega}{\m{\bm $\omega$\ubm}}
\nwc{\bmsigma}{\m{\bm $\sigma$\ubm}}
\nwc{\bmnabla}{\m{\bm $\nabla$\ubm}}
\nwc{\bmlambda}{\m{\bm $\lambda$\ubm}}
\nwc{\bmtau}{\m{\bm $\tau$\ubm}}

\nwc{\ca}{{\cal A}}
\nwc{\cao}{{\cal A}^{-1}}
\nwc{\cb}{{\cal B}}
\nwc{\cc}{{\cal C}}
\nwc{\cd}{{\cal D}}
\nwc{\ce}{{\cal E}}
\nwc{\cf}{{\cal F}}
\nwc{\cg}{{\cal G}}
\nwc{\ch}{{\cal H}}
\nwc{\ci}{{\cal I}}
\nwc{\cj}{{\cal J}}
\nwc{\ck}{{\cal K}}
\nwc{\cl}{{\cal L}}
\nwc{\clu}{{\cal L}{\cal U}}
\nwc{\cm}{{\cal M}}
\nwc{\cn}{{\cal N}}
\nwc{\co}{{\cal O}}
\nwc{\cp}{{\cal P}}
\nwc{\cq}{{\cal Q}}
\nwc{\calr}{{\cal R}}
\nwc{\cs}{{\cal S}}
\nwc{\ct}{{\cal T}}
\nwc{\cu}{{\cal U}}
\nwc{\cv}{{\cal V}}
\nwc{\cw}{{\cal W}}
\nwc{\cx}{{\cal X}}
\nwc{\cy}{{\cal Y}}
\nwc{\cz}{{\cal Z}}


\nwc{\ea}{\end{array}}
\nwc{\ee}{\end{equation}}
\nwc{\edm}{\end{displaymath}}
\nwc{\eeq}{\end{eqnarray}}
\nwc{\eeqn}{\end{eqnarray*}}
\nwc{\eeqast}{\end{eqnarray*}}

\nwc{\half}{\frac{1}{2}}

\nwc{\noi}{\noindent}
\nwc{\non}{\nonumber}
\nwc{\onehalf}{\frac{1}{2}}
\nwc{\onethird}{\frac{1}{3}}

\nwc{\p}{\partial}

\nwc{\uP}{{\em \bf Proof: }}
\nwc{\uT}{\underline{Theorem:}}









